A Multifactorial Optimization Paradigm for Linkage Tree Genetic Algorithm

Linkage Tree Genetic Algorithm (LTGA) is an effective Evolutionary Algorithm (EA) to solve complex problems using the linkage information between problem variables. LTGA performs well in various kinds of single-task optimization and yields promising results in comparison with the canonical genetic algorithm. However, LTGA is an unsuitable method for dealing with multi-task optimization problems. On the other hand, Multifactorial Optimization (MFO) can simultaneously solve independent optimization problems, which are encoded in a unified representation to take advantage of the process of knowledge transfer. In this paper, we introduce Multifactorial Linkage Tree Genetic Algorithm (MF-LTGA) by combining the main features of both LTGA and MFO. MF-LTGA is able to tackle multiple optimization tasks at the same time, each task learns the dependency between problem variables from the shared representation. This knowledge serves to determine the high-quality partial solutions for supporting other tasks in exploring the search space. Moreover, MF-LTGA speeds up convergence because of knowledge transfer of relevant problems. We demonstrate the effectiveness of the proposed algorithm on two benchmark problems: Clustered Shortest-Path Tree Problem and Deceptive Trap Function. In comparison to LTGA and existing methods, MF-LTGA outperforms in quality of the solution or in computation time.

==> Sections/Sec_Ltga.tex <==
\glsresetall
\subsection{Construct Linkage Tree}
\gls{ltga} aims to identify which variables should be treated as a dependent set of variables then agglomerative hierarchical clustering algorithms proceeds bottom-up. Hierarchical clustering algorithm to construct Linkage information between variables, then store it as a tree is called Linkage Tree. Each node in the Linkage Tree is clusters of genes is close to each other. The first stage of the algorithm considering each gene as a dependent cluster then joins two closest clusters to generate a bigger cluster until all genes are clustered into a cluster. For details is showed in Algorithm  \ref{alg:HierarchicalClustering}:

\begin{algorithm}
	Compute the proximity matrix using metric $D$.\\
	Assign each variable to a single cluster.\\
	Repeat until one cluster left:\\
	\quad Join two nearest clusters $C_i$ and $C_j$ into $C_{ij}$.\\
	\quad Remove $C_i$ and $C_j$ from the proximity matrix.\\
	\quad Compute the distance between $C_{ij}$ and all clusters.\\
	\quad Add cluster $C_{ij}$ to the proximity matrix.\\
	\caption{Hierarchical Clustering} 
	\label{alg:HierarchicalClustering}
\end{algorithm}
\renewcommand{\scalefigure}{0.35}
\begin{figure}[htbp]
	\centering
	\includegraphics[scale=\scalefigure]{Pictures/ProposedAlgorithm/hierarchicalClustering.PNG}
	\caption{The example of hierarchical clustering algorithm on 7 genes.}
	\label{fig:hierarchicalclustering}
\end{figure}
Example of hierarchical clustering in figure \ref{fig:hierarchicalclustering}.the first two closest genes $x_1$ and $x_2$ is joined into a cluster $x_1 x_2$, clusters $x_1$, $x_2$  is removed from the proximity matrix. In the next iteration, \gls{ltga} consider the distance between new cluster $x_1 x_2$ and the others cluster, then cluster two closest clusters from remaining cluster. After each generation, \gls{ltga} rebuilds the linkage tree from current population, the number of individual in  generation is large then  linkage tree represent more accurately the distribution of population.
THEM VE CLUSTER DISTANCE O DAY NUA CAC LOAI CLUSTER DISTANCE
\subsection{Crossover}
 Linkage Tree is constructed from population is used for
 

==> Table_Data/DeceptiveTrapSetup.tex <==
% Table generated by Excel2LaTeX from sheet 'TongHop_Paper'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|c|r|r|r|r|r|r|r|}
    \hline
    \multicolumn{2}{|c|}{\multirow{2}[4]{*}{}} & \multicolumn{6}{c|}{m} \\
    \cline{3-8}    \multicolumn{2}{|c|}{} & 5     & 10    & 15    & 20    & 25    & 30 \\
    \hline
    \multirow{3}[6]{*}{k} & 4     & 20    & 40    & 60    & 80    & 100   & 120 \\
	\cline{2-8}          & 5     & 25    & 50    & 75    & 100   & 125   & 150 \\
	\cline{2-8}          & 6     & 30    & 60    & 90    & 120   & 150   & 180 \\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> Table_Data/ResultsDeceptiveTrap-1.tex <==
% Table generated by Excel2LaTeX from sheet 'TongHop_Paper'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|r|r|r|r|r|r|}
    \hline
    \multicolumn{2}{|c}{} & \multicolumn{2}{|c}{\textbf{\glsentryshort{ltga}}} & \multicolumn{2}{|c|}{\textbf{\glsentryshort{mfltga}}} \\
    \hline
    \multicolumn{1}{|l|}{k} & \multicolumn{1}{l|}{m} & \multicolumn{1}{c|}{Num.Opt} & \multicolumn{1}{c|}{Num.Evals} & \multicolumn{1}{c|}{Num.Opt} & \multicolumn{1}{c|}{Num.Evals} \\
    \hline
    3     & 5     & 10 & 4,228.0 & 10 & 2783.2 \\
    \hline
    3     & 10    & 10 & 13,664.8 & 10 & 8908.8\\
    \hline
    3     & 15    & 10 & 24,552.0 & 10 & 13780.8\\
    \hline
    3     & 20    & 10 & 34,007.6  & 10 & 23434.8\\
    \hline
    3     & 25    & 10 & 52,244.0 & 10 & 28179.2\\
    \hline
    3     & 30    & 10 & 57,387.2 & 10 & 39765.2 \\
    \hline
    4     & 5     & 10 & 7706.4 & 10 & 6642.4 \\
    \hline
    4     & 10    & 10 & 25615.2 & 10 & 23587.2 \\
    \hline
    4     & 15    & 10 & 39010.8 & 10 & 38043.2 \\
    \hline
    4     & 20    & 10 & 64053.2 & 10 & 61209.2 \\
    \hline
    4     & 25    & 10 & 5021.2 & 10 & 66013.2 \\
    \hline
    4     & 30    & 10 & 111479.2 & 10 & 95200.0\\
    \hline
    5     & 5     & 10 & 20342.4 & 10 & 13900.8 \\
    \hline
    5     & 10    & 10 & 66150.0 & 10 & 49568.4 \\
    \hline
    5     & 15    & 10 & 123994.4 & 10 & 65327.2 \\
    \hline
    5     & 20    & 10 & 176378.4 & 9 & 145569.6 \\
    \hline
    5     & 25    & 10    & 231582.4 & 10    & 128116.8 \\
    \hline
    5     & 30    & 10    & 284411.2 & 10    & 196322.4 \\
	\hline
	\end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> Table_Data/ResultsDeceptiveTrap.tex <==
%\begin{ThreePartTable}
%	\begin{TableNotes}
%		\footnotesize
%		\item Num. Opt: The number of optimal solutions are found; \hspace{1cm}  Num. Eval: Number of function evaluation;
%		%		\item PIs: PI(Single task, AAL); \hspace{1cm} PIm: PI(Multi-tasks, AAL)
%	\end{TableNotes}
\begin{table}
  \centering
  \caption{Results Obtained By \glsentryshort{ltga} and \glsentryshort{mfltga}} \label{tab:ResultsDeceptiveTrap}%
    \begin{tabular}{|c|r|r|r|r|r|r|}
    \hline
     \multicolumn{3}{|c|}{}& \multicolumn{2}{c|}{\textbf{\glsentryshort{ltga}}} & \multicolumn{2}{c|}{\textbf{\glsentryshort{mfltga}}}\\
     \hline
    \multicolumn{1}{|l|}{\textbf{No.}} & 
    \multicolumn{1}{l|}{\textbf{k}} & 
    \multicolumn{1}{l|}{\textbf{m}} & 
    \multicolumn{1}{c|}{\textbf{Num.Opt}} & 
    \multicolumn{1}{c|}{\textbf{Num.Eval}} & 
    \multicolumn{1}{c|}{\textbf{Num.Opt}} & 
    \multicolumn{1}{c|}{\textbf{Num.Eval}} \\
 
    \hline
    1     & 4     & 5     & 10    & 7706.4 & 10    & 6642.4 \\
    \hline
    2     & 4     & 10    & 10    & 25615.2 & 10    & 23587.2 \\
    \hline
    3     & 4     & 15    & 10    & 39010.8 & 10    & 38043.2 \\
    \hline
    4     & 4     & 20    & 10    & 64053.2 & 10    & 61209.2 \\
    \hline
    5     & 4     & 25    & 10    & 85021.2 & 10    & 66013.2 \\
    \hline
    6     & 4     & 30    & 10    & 111479.2 & 10    & 95200.0 \\
    \hline
    7     & 5     & 5     & 10    & 20342.4 & 10    & 13900.8 \\
    \hline
    8     & 5     & 10    & 10    & 66150.0 & 10    & 49568.4 \\
    \hline
    9     & 5     & 15    & 10    & 123994.4 & 10    & 65327.2 \\
    \hline
    10    & 5     & 20    & 10    & 176378.4 & 9     & 145569.6 \\
    \hline
    11    & 5     & 25    & 10    & 231582.4 & 10     & 128116.80 \\
     \hline
    12    & 5     & 30    & 10    & 284411.2 & 10     & 196322.40 \\
    \hline
    \multicolumn{7}{r}{\begin{tiny} Num.Opt: The number of optimal solutions are found;  Num.Eval: Number of evaluations to success  \end{tiny} }\\
%    \multicolumn{7}{r}{{\tiny Num.Eval: Number of function evaluation}}\\
    \end{tabular}%
%  	\insertTableNotes
\end{table}%
%\end{ThreePartTable}


==> Table_Data/ResultsType34.tex <==
\begin{ThreePartTable}
	\begin{TableNotes}
		\footnotesize
		\item Rm: Running time of algorithms in minutes; \hspace{1cm}  Ins: Problem Instances; %\hspace{1cm} PIs: PI(Single task, AAL); \hspace{1cm} PIm: PI(Multi-tasks, AAL)
		%		\item PIs: PI(Single task, AAL); \hspace{1cm} PIm: PI(Multi-tasks, AAL)
	\end{TableNotes}
 \begin{longtable}{|c|l|r|r|c|r|r|c|r|r|r|}
	\caption{Results Obtained By E-MFEA, C-MFEA And NEA on Instances In Type 3 and Type 4} \label{tab:ResultsType34}\\
	\hline
	\multirow{2}[4]{*}{} & 
	\multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Ins}}} & 
	%E-MFEA
	\multicolumn{3}{c|}{\textbf{E-MFEA}} & 
	%C-MFEA
	\multicolumn{3}{c|}{\textbf{C-MFEA}} & 
	%NEA
	\multicolumn{3}{c|}{\textbf{NEA}} \\
	
	%Line 2 of Heading
	\cline{3-11}          &       & 
	%E-MFEA
	\multicolumn{1}{c|}{\textbf{BF}} & 
	\multicolumn{1}{c|}{\textbf{Avg}} & 
	\multicolumn{1}{p{1.3em}|}{\textbf{Rm}}& 
	%C-MFEA
	\multicolumn{1}{c|}{\textbf{BF}} & 
	\multicolumn{1}{c|}{\textbf{Avg}} & 
	\multicolumn{1}{p{1.3em}|}{\textbf{Rm}} & 
	%NEA
	\multicolumn{1}{c|}{\textbf{BF}} & 
	\multicolumn{1}{c|}{\textbf{Avg}} & 
	\multicolumn{1}{p{1.3em}|}{\textbf{Rm}}\\

    \hline
    \multirow{5}[10]{*}{\begin{sideways}\textbf{Type 3}\end{sideways}} & 6i300 & \multicolumn{1}{c|}{28672.7} & \multicolumn{1}{c|}{30356.7} & 7.38  & \multicolumn{1}{c|}{31283.6} & \multicolumn{1}{c|}{39444.1} & 1.22  & 19358.8 & 19467.0 & 0.02 \\
		\cline{2-11}          & 6i350 & \multicolumn{1}{c|}{32978.7} & \multicolumn{1}{c|}{34541.8} & 7.38  & \multicolumn{1}{c|}{78019.0} & \multicolumn{1}{c|}{87416.8} & 1.22  & 21472.8 & 21702.2 & 0.02 \\
		\cline{2-11}          & 6i400 & \multicolumn{1}{c|}{43086.1} & \multicolumn{1}{c|}{46328.2} & 10.47 & \multicolumn{1}{c|}{52463.2} & \multicolumn{1}{c|}{62720.6} & 2.05  & 29506.9 & 29677.7 & 0.02 \\
		\cline{2-11}          & 6i450 & \multicolumn{1}{c|}{51738.6} & \multicolumn{1}{c|}{55060.5} & 10.47 & \multicolumn{1}{c|}{124525.9} & \multicolumn{1}{c|}{137183.6} & 2.05  & 35866.3 & 36124.5 & 0.02 \\
		\cline{2-11}          & 6i500 & \multicolumn{1}{c|}{61227.4} & \multicolumn{1}{c|}{69324.1} & 5.88  & \multicolumn{1}{c|}{143220.7} & \multicolumn{1}{c|}{153699.3} & 2.93  & 37711.6 & 38045.9 & 0.02 \\
		    \hline
		    \multirow{10}[20]{*}{\begin{sideways}\textbf{Type 4}\end{sideways}} & 4i200a & 329844.5 & 393407.0 & 0.07  & 1058533.6 & 1150968.4 & 0.02  & 97959.6 & 102256.3 & 0.00 \\
		\cline{2-11}          & 4i200h & 215812.7 & 248321.3 & 0.07  & 604259.8 & 652916.9 & 0.02  & 87675.3 & 89628.9 & 0.00 \\
		\cline{2-11}          & 4i200x1 & 239439.4 & 258423.4 & 0.07  & 621807.6 & 680006.8 & 0.02  & 123669.7 & 125782.7 & 0.00 \\
		\cline{2-11}          & 4i200x2 & 226820.7 & 254560.0 & 0.07  & 631471.0 & 671268.7 & 0.02  & 114012.3 & 116256.5 & 0.00 \\
		\cline{2-11}          & 4i200z & 259796.7 & 284456.1 & 0.40  & 265010.4 & 284466.7 & 0.05  & 131683.5 & 133873.8 & 0.00 \\
		\cline{2-11}          & 4i400a & 834356.4 & 948781.5 & 0.40  & 4681600.4 & 5013170.5 & 0.05  & 217171.4 & 227530.6 & 0.02 \\
		\cline{2-11}          & 4i400h & 655591.7 & 713631.1 & 5.15  & 2602030.7 & 2808230.9 & 3.05  & 257954.4 & 260916.0 & 0.02 \\
		\cline{2-11}          & 4i400x1 & 569429.8 & 667408.9 & 5.15  & 2481894.5 & 2668551.2 & 3.05  & 188786.2 & 191694.7 & 0.02 \\
		\cline{2-11}          & 4i400x2 & 570171.7 & 639480.4 & 5.50  & 2478070.1 & 2659442.4 & 3.13  & 159254.8 & 163222.8 & 0.02 \\
		\cline{2-11}          & 4i400z & 588799.3 & 674446.0 & 5.50  & 2512497.8 & 2723834.3 & 3.13  & 221460.6 & 225096.3 & 0.02 \\
    	\hline
	  \insertTableNotes	  
	\end{longtable}%
\end{ThreePartTable}
